A Formalization of Elementary Linear Algebra: Part I

This is the first installment of an exposition of an ACL2 formalization of elementary linear algebra, focusing on aspects of the subject that apply to matrices over an arbitrary commutative ring with identity, in anticipation of a future treatment of the characteristic polynomial of a matrix, which has entries in a polyniomial ring. The main contribution of this paper is a formal theory of the determinant, including its characterization as the unique alternating n-linear function of the rows of an non matrix, multiplicativity of the determinant, and the correctness of cofactor expansion.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Gamboa and Manolios (Eds):\\
ACL2 Workshop 2025\\
EPTCS 423, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.423.1}{10.4204/EPTCS.423.1}}

